LLM Censorship: A Machine Learning Challenge or a Computer Security Problem?

Large language models (LLMs) have exhibited impressive capabilities in comprehending complex instructions. However, their blind adherence to provided instructions has led to concerns regarding risks of malicious use. Existing defence mechanisms, such as model fine-tuning or output censorship using LLMs, have proven to be fallible, as LLMs can still generate problematic responses. Commonly employed censorship approaches treat the issue as a machine learning problem and rely on another LM to detect undesirable content in LLM outputs. In this paper, we present the theoretical limitations of such semantic censorship approaches. Specifically, we demonstrate that semantic censorship can be perceived as an undecidable problem, highlighting the inherent challenges in censorship that arise due to LLMs' programmatic and instruction-following capabilities. Furthermore, we argue that the challenges extend beyond semantic censorship, as knowledgeable attackers can reconstruct impermissible outputs from a collection of permissible ones. As a result, we propose that the problem of censorship needs to be reevaluated; it should be treated as a security problem which warrants the adaptation of security-based approaches to mitigate potential risks.

==> all.tex <==
\section{Abstract}
Large language models (LLMs) display advanced capabilities to follow instructions. When coupled with their sensitivity to alterations in input prompts and tool access, this poses substantial concerns regarding potential misuse. In efforts to counteract various malicious actors, companies have adopted ad hoc censorship strategies. For instance, ChatGPT presently declines to provide guidance on constructing a firearm at home. Nevertheless, these preventive measures are not foolproof, as an adversarial prompt still evokes a response. In this work, we introduce a framework to articulate the design of a secure LLM-based system. An integral component of the framework is censorship: a collection of mechanisms restricting inputs and outputs to a set of constraint-satisfying strings. Constraints are specified by model providers and can be broken down into two types—semantic and syntactic. We characterise impossibility results of verifying semantic properties, such as whether or not the model output contains malware, and propose prompts templates, a method that employs strong syntactic constraints to enable the design and practical verification of secure LLM-based systems. Our framework offers a promising path towards trustworthy deployment of LLM-based systems

\section{Introduction}
In recent years, Large Language Models (LLMs) have made remarkable strides in various tasks such as text generation, problem solving, and instruction following~\cite{}, driven by advances in prompt engineering and Reinforcement Learning with Human Feedback (RLHF)~\cite{ziegler2020finetuning, ouyang2022training}. These developments have significantly enhanced LLMs' ability to understand instructions, produce outputs preferred by humans, and have enabled simple and smooth user interaction with LLMs. Additionally, the integration of external tools and applications (with LLMs), including APIs, external memory and web retrieval, and code interpreters, has further expanded their capabilities, accuracy, and practicality~\cite{}.

However, as the popularity of LLMs grows, concerns have arisen regarding their safety and security risks, particularly with regards to potential misuse by malicious actors. These risks encompass a wide range of issues, such as social engineering and data exfiltration~\cite{greshake2023youve, weidinger2022taxonomy}. Thus, efforts have been made to fine-tune LLMs using RLHF and similar methods to mitigate the generation of unsafe or harmful content~\cite{openai2023gpt4}. Nevertheless, the brittleness of LLMs persists, and well-crafted prompts can still bypass these defenses~\cite{Jailbreak}. Recent theoretical findings~\cite{wolf2023fundamental} even suggest that there exist prompts that can trigger {\em any behaviour} achievable by an LLM with high probability.

To address these limitations, some approaches have focused on external censorship tools. For instance, OpenAI proposed training language models to classify and censor model outputs~\cite{markov2023holistic}, while Nvidia's NeMo Guardrails toolkit allows model providers to specify constraints on user inputs and model outputs, and employ LLMs to verify if the constraints are satisfied~\cite{Chockalingam_Varshney_2023}. However, these methods, at best, serve as deterrents and lack provable safety or security guarantees. 


In this paper, we aim to identify the theoretical challenges associated with censorship and present a framework that fosters further research in the design of safe and secure LLM-based systems.  To shed light on the limitations of censorship, we first distinguish between two types: semantic and syntactic. Semantic censorship aims to filter strings based on their underlying meaning, while syntactic censorship focuses on specific content or patterns within the string. We demonstrate the impossibility of achieving nontrivial semantic censorship for LLMs capable of processing and producing program descriptions as output, presenting three impossibility results by describing worst-case attacks.

Informed by these challenges, we propose a general framework that facilitates the understanding, discussion, and design of secure LLM-based systems. This framework categorises participating agents, including LLMs, model users, and external tools, into trusted and untrusted groups where information can be exchanged freely amongst agents in the same group. However, to ensure security, strong syntactic censorship is required to control information flow from untrusted sources to trusted agents.

Finally, we discuss the implications of our results and proposed framework. We illustrate how the framework enhances the understanding of the successes and limitations of a recently proposed defence against prompt injection attacks. Additionally, we present a more general defence strategy that utilises a collection of prompt templates, enabling untrusted models to specify relevant parts of their output as variable tokens. Censorship is performed using a classifier to select constraint-satisfying prompt templates based on the untrusted output, and verification can then be achieved through exhaustive search.

To summarise, our contributions are as follows
\begin{enumerate}
    \item In \cref{sec:Secure Framework} we present a general framework for understanding the design of secure LLM-based systems, identifying all relevant components and making clear the role of Censorship within the framework. Furthermore we distinguish and define different types of censorship, such as semantic and syntactic in \cref{sec:semantic vs syntactic}
    \item We provide several results demonstrating limitations of semantic censorship, namely Undecidability \cref{sec:Undecidability}, Obfuscation \cref{sec:Encryption}, and Mosaic Prompts \cref{sec:Mosaic}
    \item We provide a discussion \cref{sec:defenses} on the implications of our results and how our framework can be utilized for the design of secure LLM-based systems through strong syntactic censorship in the form of prompt template classification 

\end{enumerate}

\section{Framework for Secure LLM-Based systems} \label{sec:Secure Framework}
Properly establishing a framework of LLM-Based system interaction requires identifying all 
ways the system interacts with the world. We propose to distinguish all external interactions with a system in terms of two categories of agents: Users and Receivers. 
\begin{itemize}
    \item \textbf{(Users):} The set of Users $U := \{u_1, u_2,\dots, u_k\}$ are external agents who provide inputs to an LLM-Based system. These can include an individual asking a question, and an email/website that is read by the LLM-Based system.
    \item \textbf{(Receivers):} The set of Receivers $R := \{r_1,r_2,\dots,r_j\}$ are external agents that receive outputs from the LLM-Based system. These can include a user reading a response to their question, or a tool which deletes an email if instructed. 
\end{itemize}   
\begin{definition}[\textbf{LLM-Based Model}]
We define an LLM-Based Model $F(M,C)$ to consist of a collection of models $M := \{m_1,m_2,\dots,m_n\}$ and controller $C$. Models $m$ take strings as input and produce strings as output. At least one model must be a LLM, and other models can include software tools such as Python interpreters. The controller facilitates interactions between the various components of the model, functioning as an interface between LLMs and tools. (possibly unnecessary...)
\end{definition}
To design a secure LLM-Based system one must take into account both the LLM-Based model as well as its external interactions with users and receivers. We assume that all security risks posed by an LLM-Based system manifest through its external interactions, in particular from the outputs to receivers. 

As within certain settings some users or receivers may be assumed to pose no security risks, an LLM-Based system can be divided into two groups, \emph{trusted} and \emph{untrusted}.  
\begin{itemize}
    \item (\textbf{Trusted:}) Users, models, and receivers that are \textit{trusted} are those assumed by the model designer to produce outputs that pose no security risk and take inputs that pose no security risk as applicable. (do we want to capture something like "intentionality" where accidents/bugs/natural adversarial examples are permitted to be trusted even if they pose a security risk?)
    \item (\textbf{Untrusted:}) Users and models that are \textit{untrusted} are those whose outputs are assumed to pose a possible security risk, whereas untrusted receivers are receivers who can accept input from an untrusted source without a possible security risk. As models are assumed unable to self-censor, any model exposed to input from an untrusted source is untrusted. 
\end{itemize}

Finally, to allow for information from untrusted sources to still reach trusted models or receivers, Censorship mechanisms can be employed. Informally, Censorship mechanisms are methods for ensuring that a given string satisfies certain constraints set by the model designer so as to introduce no security risks if provided as input to a given trusted model or receiver. Censorship is discussed in greater detail in the following section. 

\begin{definition}[\textbf{Secure LLM-Based System}]
We define a Secure LLM-Based System system $S(F,U,R)$ where $F(M,C)$ is an LLM-Based model. The collections of users $U$ and receivers $R$ are labelled as \textit{trusted} or \textit{untrusted} depending on the possibility of security risks. At every instance of execution of the LLM-Based model based on user input, model $m \in M$, with exception of censorship mechanisms, are labelled \textit{untrusted} if they accept input via the controller $C$ from an untrusted source or may produce \textit{untrusted} output regardless, and \textit{trusted} otherwise. Censorship mechanisms can be applied to the output of an untrusted source to create an input to a trusted model or receivers. All users, models, and receivers are termed agents. 
\end{definition}
\section{Censorship}
Performing censorship in order to enable for an exchange of information from untrusted to trusted agents relies on verifying whether a given string satisfies a collection of constraints $c$ set by model designer based on perceived potential security risks. We define constraints in terms of formal languages. 

We assume that all inputs and outputs take the form of strings defined over a token vocabulary $\Sigma$ with $\Sigma^*$ the Kleene star of $\Sigma$. 
\begin{definition}[\textbf{Constraints:}]
    A collection of security-ensuring properties $c_{sa}$ of string outputs of an untrusted source $s$ with respect to trusted agent $a$ are the \textit{constraints} on untrusted source $s$ with respect to trusted agent $a$. 
\end{definition}

Security-ensuring properties are a collection of properties of strings determined by the model designer which collectively ensure a string possessing all those properties does not induce any security risk when provided to a trusted agent. It is the responsibility of the model designer to verify that these properties are in fact sufficient to prevent security risks. We discuss a possible method for verification in \cref{sec:defenses}.

The definition of properties and constraints provided is very general. To enable us to make meaningful statements on limitations of censorship we draw inspiration from properties of program descriptions to derive a useful distinction. 
\subsection{Semantic Versus Syntactic Censorship}\label{sec:semantic vs syntactic}
Censorship relies on verification if certain constraints are satisfied, in other words, verification if strings possess certain properties. We distinguish between two types, \textit{semantic} properties and \textit{syntactic} properties. Informally, semantic properties that have to do with the meaning of a string, in the case of program descriptions with the behaviours of the program. Syntactic properties are non-semantic properties, usually properties of the string such as patterns of tokens that occur or structural properties of the sting itself. 


\subsection{Semantic Properties}
Defining the "meaning" of a string formally is outside of the scope of this work. Instead we first focus on strings that describe programs, after which we add another property to allow for a definition for semantic properties which encompasses all strings. 

Informally, one can think of a semantic property of a program description as a property about the functional behaviour of the program it describes. By functional behaviour, we mean \textit{what the program does} rather than \textit{how it does it}. Under this notion, a program halting is a functional behaviour whereas a program running for 100 steps before halting is not.
\begin{definition}[\textbf{Program Description Semantic Properties}]\label{def:sem1}
    For a given program (Turing machine) description $\langle P \rangle$ of a program $P$, its semantic properties are the properties of the language $L(P)$ recognised by $P$.
\end{definition} 

To extend the notion of semantic properties to general strings and capture the intuition that an encrypted string still possesses properties of it's decryption, we propose the following definition.
\begin{definition}[\textbf{String Semantic Properties}]\label{def:sem2}
    A semantic property of a string $w$ is a property which is preserved under arbitrary invertible transformation $g: \Sigma^* \to \Sigma^*$ assuming the inverse mapping $g^{-1}$ is known
\end{definition}
\begin{example} In the setting where a model user $u$ provides $F$ with input $x$ requesting for a program description $\langle P \rangle$ of a keylogger returned as $g(\langle P \rangle)$ for specified encryption method $g$. If the user is also the final output receiver, they can recover $\langle P \rangle$ by decrypting $g(\langle P \rangle)$ using $g^{-1}$; if $F(x) = g(\langle P \rangle)$ then this encrypted output still possesses the same semantic properties as the malware encoding $\langle P \rangle$.
\end{example}  
\begin{theorem}[Semantic Property Extension]
    All semantic properties of program descriptions under \cref{def:sem1} remain under \cref{def:sem2}.  
\end{theorem}
\textit{Sketch of Proof}: Given an encoding of a program $\langle P \rangle$, one can recover the program $P$ by providing the encoding $\langle P \rangle$ to a Universal Turing Machine $T_1$ as input, which it uses to emulate program $P$. One can consider another Universal Turing Machine $T_2$ which first applies the transform $g^{-1}$ before running $T_1$ on the input. Then, the program emulated by $T_2$ when provided with $g(\langle P \rangle)$ is the same program $P$. Both program descriptions describe identical programs which recognise the same language.
\begin{remark}
    \cref{def:sem2} does not intend to broadly capture what is commonly thought of as semantic properties, for example the common property of two different sentences which have the same meaning. While many distinct strings provided to an LLM may be "interpreted very similarly" and induce very similar distributions over outputs, this does not necessarily result in a significant limitation for censorship. For example if one of the problematic strings is identified it could be utilised as an anchor to identify strings which induce similar output behaviour as part of a censorship mechanism.
\end{remark}
\subsection{Syntactic Properties}
Unlike semantic properties, which can be preserved under arbitrary invertible translations $g$, syntactic properties cannot. Whereas semantic properties aim to capture properties of the content of a string, syntactic properties aim to capture properties of the string itself.
\begin{definition}[Syntactic Properties]
    A syntactic property of a string $w$ is a property which is not preserved under arbitrary invertible transformations $g: \Sigma^* \to \Sigma^*$ even if $g^{-1}$ is known.
\end{definition}
\begin{example}
    The property of a program description containing the substring "while" would not be preserved under a translation $g$ that replaces "while" with another symbol. (better/more examples?)
\end{example}
By their nature, Syntactic constrains are easily verifiable relative to semantic properties, an intuition which we demonstrate through theoretical limitations of semantic censorship in \cref{sec:Undecidability} and \cref{sec:Encryption}. While censorship using syntactic properties can feel limiting as they fail to capture many abstract properties we seek to censor, in practice these properties can be useful. In fact, we rely on strong syntactic properties as part of the prompt templates defense described in \cref{sec:defenses}.
Having defined two types of properties of strings that determine which strings are censored or not, we define two types of censorship mechanisms, local and global that determine how strings are censored. 
\subsection{Local and Global Censorship}
We consider two types of potential censorship mechanisms: \textit{Local} and \textit{Global}. Local censorship mechanisms filter inputs from untrusted sources by allowing constraint satisfying strings to pass to a trusted agent freely and converting constraint violating strings to a constraint satisfying one before passing them on. Global Censorship mechanisms on the other hand focus on solely on the censorship of any inputs to trusted receivers from untrusted sources, and can utilise all intermediate model outputs and user inputs that were used to produce the final output to the receiver.

To define censorship mechanisms formally, we describe them in terms of  set of constraints $c$, user $u$, and model $m$ we use $L_c \subset L_{m,u}$ to denote the intersection of the set of constraint satisfying strings with the set of possible model outputs;  $L_c' = L_{m,u} \setminus L_c$ is its complement
\begin{definition}[Local Censorship]
A Local censorship mechanism is a model $m \in M$ which receives input from untrusted source $s$ and outputs to trusted agent $a$ 
\begin{align*}
    m(x) = 
    \begin{cases}
        x & \text{if } x \in L_c\\
        x_c & \text{otherwise}
    \end{cases}
\end{align*}
where $x_c \in L_c$ and may or may not depend on $x$. 
\end{definition}

\begin{remark}
Local censorship mechanisms always convert untrusted outputs to trusted inputs by ensuring they satisfy necessary constraints. 
Interactions between trusted agents are always assumed to satisfy necessary constraints, and interactions between untrusted agents have no constraints. 
\end{remark}

\begin{remark}
In order to ensure security, for any local censorship mechanism, all elements $x \in L_c$ must be such that any possible constraints on downstream trusted model outputs are maintained without the need for additional censorship mechanisms, that is they need to satisfy the requirements necessary to be treated as if they came from a trusted model or user.
\end{remark}
\begin{definition}[Global censorship]
Global censorship mechanisms take into account all inputs and outputs to determine if the output $F(x)$ needs to be censored based on constraints $c$. 
\end{definition}

We do not consider censorship mechanisms that rely on intermediate representations of LLMs as these are not interpretable and would result in unreliable security measures, however if possible and applicable, global censorship mechanisms could have access to intermediate states of tools used.

\section{Undecidability and Practical Implications}\label{sec:Undecidability}
\subsection{Classical Results}
Recall Rice's Theorem, a well-known result in the theory of computation:
\begin{theorem}[Rice's Theorem, Informal]
    Any nontrivial property about the language recognised by a Turing machine is \textit{undecidable}.
\end{theorem} 
In simple words, the above states that the problem of determining any non-trivial semantic property of a program $P$ is \textit{undecidable} and therefore no general algorithm exists. A well known corrolary of this theorem is towards establishing Undecidability of the halting problem.

\begin{corollary}[Undecidability of the Halting Problem]\label{cor:Halting}
    The language given by $\{\langle P, x\rangle | \text{ program } P \text{ halts on input }x \}$ is undecidable 
\end{corollary}
The specific property of the language in question is that it consists of strings describing programs that halt on a given input. The consequence of \cref{cor:Halting} is that one cannot have a general algorithm that predicts whether or not a program stops on a given input. 

For any semantic property $q \in c_{sa}$ that is among the constraints imposed on program descriptions, e.g. it does not describe a computer virus, the following corollary applies. Note 
\begin{corollary}[Undecidability of Semantic Censorship]
    For nontrivial property $q$, the language given by $\{\langle P \rangle | \text{ program } P \text{ has property q}\}$ is undecidable.
\end{corollary}
For a property to be nontrivial, there must exist programs with and without this property. Thus, no general algorithm can exist that predicts whether or not a program description satisfies censorship constraints or not.

\par 
We conclude that a local censorship mechanism that relies on semantic constraints on outputs produced by a model, inputs provided by a user, or outputs to a receiver cannot exist. Naturally the same result implies that a global censorship mechanism relying on semantic constraints cannot exist either. 
\begin{remark}[Practical Limitations of Theory]
In practice, we deal with 
\begin{enumerate}
    \item Bounded inputs and outputs
    \item Bounded computer memory
\end{enumerate}
Thus, Turing machines do not exist in practice and the undecidability result given by Rice's theorem doesn't strictly hold in the real world. 
\end{remark}
Despite the practical limitations, verifying semantic properties of programs remains an incredibly challenging task in practice. Malware and virus detection are two examples where a detection is eternally trying to keep up with development of new attacks and detection evasion methods. A common property of many detection evasion methods is encryption \cite{caviglione2020tight}, which inspired our next impossibility result for censorship. 

\section{Encryption}\label{sec:Encryption}
We describe an impossibility result for non-trivial output censorship according to semantic constraints, and then discuss practical implications. 

For an LLM-based system $S(F,U,R)$ system we assume that each receiver $r$ has possession of a finite set of translation schemes $G_r := \{(g_1,g^{-1}_1), (g_2,g^{-1}_2), \dots, (g_k,g^{-1}_k)$ which they can use to interpret outputs received. For convenience we assume that for all external tool receivers $r$, $G_r = \{g_r\}$ where $g_r$ is an encoding translation scheme known to the model provider. 
\subsection{Impossibility of Semantic Censorship}
The following impossibility result relies on a key assumption of the LLM-based models capabilities to follow instructions and compute mappings over strings. In particular, it requires that some output of a model that passes through a censorship mechanism could have been transformed by an arbitrary mapping over strings $g$. 
\begin{wrapfigure}{r}{0.4\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/try1.png}
\end{wrapfigure}

Specifically, for a secure LLM-based system $S(F,U,R)$ and input $x$ provided by untrusted user $u \in U$, there is a path of inputs and outputs taken before a final output is produced for a trusted receiver $r \in R$. Unless the user input is immediately censored before being provided to a trusted model, there exists a non-empty set of exchanges where an output of an untrusted model must pass through a local censorship mechanism. We assume that for one of these outputs, its length is bounded by $n$ and the programmatic capabilities of the model up to that point are sufficient to compute any bijective map over strings of length bounded by $n$. (how to state this formally in an assumption block? I'm not stating turing completeness, since that doesn't exist in practice...)
\begin{assumption}\label{ass:1}
    The programmatic capabilities of the path through an LLM-based system including the model whose output goes through a censorship mechanism are sufficient to compute any bijection over strings of length at most $n$ 
\end{assumption}

Many tools employed by models satisfy this assumption, as tools such as Python interpreters enable one to execute such mappings.
\begin{theorem}[Impossibility of Local Semantic Censorship of model outputs] \label{thm:1}
    Let $S(F,U,R)$ be an LLM-Based system. Let $r \in R$ be a trusted receiver that possesses an unknown set of translation schemes $G_r$ and $m' \in M$ a local censorship mechanism between an untrusted model $m$ and trusted agent $a$. For a message of length at most $n$, if \cref{ass:1} holds then nontrivial local semantic censorship is impossible, that is $L_{c_{ma}} \in \{\emptyset,L_{m,u}\}$. 
\end{theorem}
\textit{Sketch of Proof}: There exist bijections over strings which map strings that do not satisfy constraints satisfying to strings that do. Any such bijection may be among the the set of translation schemes $G_r$ possessed by the receiver $r$ and any string in the semantic constraint satisfying language $L_{c_{ma}}$ may have the same semantic content as a string that does not satisfy semantic constraints leading to a contradiction.
\par
Thus, without any knowledge of translation schemes possessed by the receiver makes verification of non-trivial semantic constraints using based only on the output string generally impossible. When $r$ is an external tool, it can be usually assumed that the set $G_r$ is known to the censorship mechanism as it is known to the model designer when the system is designed or is common knowledge, in which case the impossibility result does not necessarily hold.
\subsection{Encryption}
One potential approach for adversaries to circumvent censorship in LLM systems is through encryption. Encryption methods employ algorithms such as Stream ciphers, which combine string characters with a binary secret key through XOR operations. By using a codebook like Unicode, which assigns a unique binary representation for each character, encryption can be achieved. The security of a Stream Cipher depends on the length and randomness of the secret key used.

LLMs are pretrained on extensive datasets and are likely to have learned common encryption methods and various codebooks. As a result, users can communicate only the secret key to the model alongside instructions on how to apply the encryption algorithm to produce an encrypted output.

To establish a secret key without public disclosure, users can employ the Diffie-Hellman key exchange, which securely exchanges keys over an insecure communication channel. Even with global censorship mechanisms in place, determining the secret key and decrypting the encrypted output would be computationally difficult.

In some cases, if the key is backdoored into an LLM, the user would not even need to communicate the key to the model. A user could provide a trigger to the model to recall and apply the secret key, akin to how detecting whether or not a canary string was memorized by a model. The model can employ One-Time pad encryption without revealing the secret key that was backdoored into it. In such instances, deducing the encryption algorithm or its inverse becomes impossible.

Adversaries can further complicate detection by employing steganography methods, hiding encrypted data within normal data. Syntactic censorship methods may impose constraints to detect encrypted outputs, but users can instruct the model to apply obfuscation techniques, such as renaming variables and functions or adding junk code, to bypass such censorship.

Considering these encryption-based evasion methods, it becomes evident that effectively censoring LLMs can be as challenging as the ongoing task of malware detection. Furthermore, LLMs require censorship of not only program encodings but also natural language outputs, adding an additional layer of complexity.

Next we introduce another unique security challenge for LLM-based systems arising due to the capability of users to recover constraint violating outputs through the composition of benign outputs generated in separate contexts.

\section{Compositional Evasion/Mosaic Prompts/Payload Splitting}\label{sec:Mosaic}
\subsection{An Example of a Mosaic Prompt}
We leverage the principle of compositionality to argue that users with knowledge of a structure $T$ corresponding to some potential program description $w \in L_{c^s}'$ could construct $w$ by acquiring expressions $e_i \in L_{c^s}$ from the model $F$ to be combined by $T$ so as to recover $w$.

\begin{myenv}{Example: Keylogger}
For example, a user may know, or perhaps learn from the model $F$, that a malicious keylogging program can be composed of phishing email that contains requests a user to download a keylogger, a program that logs keystrokes and saves them to a local file (the keylogger), and a program that sends the contents of that file to a remote server via email.

Using this knowledge of the structure $T$ of the keylogger, the user $U$ can provide three separate inputs $(x_1,x_2,x_3)$ to the model $F$ in three separate contexts:
\begin{description}
    \item[\textbf{[Prompt 1]:}]  Generate of a sample email from a fake company requesting the recipient to download an attached file
    \item[\textbf{[Prompt 2]:}] Generate a function that logs keystrokes made on a device and saves them to a local file
    \item[\textbf{[Prompt 3]:}] Generate a function which sends the contents of a local file to a remote server via email. 
\end{description}
\end{myenv}

While each individual component is generally benign and likely would not violate any semantic constraints, the user recovers a malicious keylogger through $T(o_1, o_2, o_3)$ where $o_i = F(x_i)$. We refer to this attack as compositional evasion (is there a nicer/more illustrative example I could use instead and is the name good?)



\subsection{General Formulation of Mosaic Prompt}

\begin{definition}[Mosaic Prompt]
    The principle of compositionality broadly states that the semantics of a complex expression are determined by its structure and semantics of its constituents \cite{sep-compositionality}.
\end{definition}

We note that there can exist strings $w \in L_{c^s}'$ which can be decomposed into expressions $e_i \in L_{c^s}$ and structure $T$ where $w = T(\{e_1,e_2,\dots,e_n\}$. This becomes evident as any complex expression can always be decomposed into atomic units and structure $T$.

In the context of program descriptions, the structure $T$ is determined by the syntax of the programming language and the expressions $e_i$ may themselves be complex expressions that can be further decomposed or atomic expressions such variables or mathematical operators. Assuming that all atomic expressions in code $e \in L_{c^s}$ and there exist program descriptions $w \in L_{c^s}'$ it is clear that our claim holds true.

\subsection{Challenges of Defending against Mosaic Prompts}

\begin{wrapfigure}{r}{0.5\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/try2.png}
\end{wrapfigure}

Defending against such compositional evasion methods is often infeasible, as the censorship mechanisms do not have knowledge of the broader context of which individual subexpressions $e_i$ are a part of. Each subexpression is produced within a separate context window for the model $F$, thus other subexpressions and structure $T$ which reflect the broader context are unknown. 

Mitigating such attacks relies on significantly reducing the capabilities and usefulness of the model $F$, so as to make it unable to provide any subexpressions $e_i$ that could be recombined to create something that violates semantic constraints. As any complex expression can be decomposed into atomic units and structure $T$, it is unreasonable to conclude that a model should not output anything; outputting atomic units any new or useful information to the user who already knows $T$. 

Still, for ``simple enough'' structures $T$ and ``complex enough'' subexpressions $e_i$, it is reasonable to conclude that the model $F$ can be instrumental in helping a user acquire outputs which pose substantial real world security risks.  These attack should not be overlooked, especially when the abstract structure $T$ can also be learnt from the model.

\section{Discussion}\label{sec:defenses}
In this section we discuss the implications of our limitations and guiding principles for designing practical and secure models.  
\subsection{Implications of limitations (TODO...)}
This section will contain discussion of importance of syntactic constraints and addressing the major challenge of verifying that constraints are defined so as to certifiably mitigate potential risks considered. Global censorship mechanisms may also be desirable but can be challenging to verify/certify. Concede that compositional evasion is something that cannot be fully secured against and that this should guide decision making process of whether or not to deploy models for which compositional evasion could lead to significant risks, factoring in things such as assumptions on the adversary needed for significant risks to be a concern. Note that if the set of possible model outputs is small (e.g. fixed set of classes), one could verify whether or not compositional evasion could pose a risk and what assumptions on the adversary would be needed by considering all possible combinations of model outputs. In settings where this verification is hard, stress the importance developing otherwise secure models. 

\subsection{Quarantined model and Prompt templates}
We discuss a recently proposed technique for ensuring security proposed in \cite{willison_2023} as a special case of our framework, and propose a general and practical approach for construction of secure models. The defence assumes the setting in which there exists a trusted user (e.g. an individual requesting an LLM assistant to read and respond to an email), and an untrusted user (e.g. creator of contents of an email) and correspondingly a trusted, privileged LLM $m_p$ and an untrusted, quarantined LLM $m_q$. Furthermore, the controller $C'$ is a software which handles interactions between users, LLMs, and external tools. In the described defence, $C'$ provides trusted user input to $m_p$, executes instructions provided by $m_p$, provides instructions to $m_q$, stores outputs of $m_q$ and provides censored representation to $m_p$ in the form of variable names. We note that within our framework this controller $C'$ plays the role of tool models and censorship mechanisms $m$ alongside that of the controller $C$. An example of how this Dual LLM framework would operate is provided in \cite{willison_2023} 
\begin{myenv}{Example: Dual LLMs}
\begin{itemize}\label{DualLLM_example}
    \item \textbf{User}: Summarize my latest email
    \item \textbf{Controller}: Passes the user’s request to the Privileged LLM
    \item \textbf{Privileged LLM}: Run action \texttt{fetch\_latest\_emails(1)} and assign to \texttt{\%VAR1}
    \item \textbf{Controller}: Runs that action—fetching the latest email—and assigns the result to a variable called \texttt{\%VAR1}
    \item \textbf{Privileged LLM}: Run action \texttt{quarantined\_llm('Summarize this: \%VAR1')}
    \item \textbf{Controller}: Trigger Quarantined LLM with that prompt, replacing \texttt{\%VAR1} with the previously fetched email content
    \item \textbf{Quarantined LLM}: Executes that unsafe prompt and returns the result
    \item \textbf{Controller}: Store result as \texttt{\%VAR2}. Tell Privileged LLM that summarization has completed.
    \item \textbf{Privileged LLM}: Display to the user: Your latest email, summarized: \texttt{\%VAR2}
    \item \textbf{Controller}: Displays the text "Your latest email, summarized: ... \texttt{\%VAR2} content goes here ..." to User (who is also the receiver)
\end{itemize}
\end{myenv}
Our proposed framework allows us to identify key properties underlying the effectiveness of this approach as well as characterize its vulnerabilities. We propose a natural generalization of the Dual LLMs method that allows for greater flexibility in model usage while providing the same, if not stronger security guarantees by handling settings in which all users are untrusted or uncensored outputs from untrusted models pose should not be received by receivers. The security of the Dual LLMs proposal relies on three key properties, 
\begin{enumerate}
    \item Models $m$ are separated into trusted and untrusted depending on whether they receive untrusted input, either from users or other untrusted models
    \item Untrusted models $m$ have restricted tool access, namely they can only utilise other "untrusted" tools that pose no security risks or introduce further vulnerabilities such as private data access or perform outbound actions
    \item Trusted models $m$ can accept input from untrusted sources only if the input is properly censored, i.e. it poses no security risk and is therefore trusted. This is achieved by restricting inputs to a relatively small fixed set of possible inputs such as variable names which are either assumed, or more properly verified, to pose no risk.
\end{enumerate}
It is clear that these key properties are core elements of the our proposed general framework of model censorship. We find that the Dual LLMs proposal is a special case of our general framework with the design choices of the primary user referred to as "User" serving the role of a trusted user as well as an untrusted receiver, the received email is an untrusted user, and censorship is achieved through local censorship mechanisms which force inputs to $m_p$ from $m_q$ to satisfy syntactic constraints of being a predefined variable name. In \cite{willison_2023} it was argued that in the example setting \cref{DualLLM_example}, social engineering is still a potential threat that poses security risks as the receiver still receives uncensored output from an untrusted model via the contents of \%VAR2. We find that this risk exists simply because the of the implicit design choice of an untrusted receiver, highlighting the importance behind such design choices.
\par 
From our proposed framework, building a secure model consists of design choices regarding designating trusted and untrusted users, models, and receivers, as well as constraints $c$ to be imposed by censorship mechanisms. As for general desired constraints $c$, certifying that Global censorship mechanisms ensure final outputs satisfy $c$ is hard or may result in overly restrictive censorship, we instead propose to utilise local censorship mechanisms that bridge untrusted and trusted agents. In particular, we propose strong syntactic constraints in the form of prompt templates. 
\par 
Prompt templates are prompts with variable name tokens, where variables correspond to parts of untrusted model outputs that are stored in external memory. A censorship mechanism can consist of a classifier which takes in an untrusted input $x$ to select the most appropriate prompt template from a fixed collection of options. Given the prompt template, an untrusted model could be employed to generate appropriate values for the variables using $x$, with these values stored in external memory and utilised by the controller $C$ as necessary. The output of the censorship mechanism to a trusted model or receiver would consist of the prompt template with variable name tokens. For settings where the trusted model or receiver require the values stored in the variables (e.g. when the final output is provided to a receiver), a classification (or in some cases if appropriate, regression) model could be provided with the corresponding variable values by the controller $C$ which it would use to select the most appropriate output from a constrained set of possible outputs.
\par 
Due to the strong syntactic constraints imposed by the local censorship mechanisms, the finite collection of possible inputs to a trusted model from an untrusted model or user could be small enough to exhaustively validate as producing constraint satisfying final outputs. For final outputs provided to a trusted receiver, constraints may be lenient enough to allow for verifying security of outputs without exhaustively verifying all possible variable substitutions in order to certify that constraints are satisfied.
\par 
The Language Model Programming framework and Language Model Query Language introduced in \cite{beurer2022prompting} could provide a practical and flexible approach for implementation. (discuss this more? Mention in conclusion?)
